Loi de Weyl presque sure pour un systeme differentiel en dimension 1

We consider quite general differential operators on the circle with a small random lower order perturbation. We embrace two points a view, the semiclassical and the high energy limits. We show (a) in the semiclassical limit, that the eigenvalues inside a subdomain of the pseudospectrum are distributed according to a Weyl law with a probability close to 1, (b) that the large eigenvalues obey a Weyl law almost surely.

==> ashautefrequence2.tex <==
Soit $l^{\omega}(w)$ la fonction rendant holomorphe
$e^{\frac{1}{h}l^{\omega}}\det E_{-+}^{\omega},$ 
et $k^{\omega}=\frac{1}{h} \partial_{w}l^{\omega},$
où
\[k_{w}=-\mathrm{tr}\, ((\partial_{\bar{w}}R_{+})E_{+}^{\delta}+
E_{-}^{\delta}(\partial_{\bar{w}}R_{-})).
\]
Le corollaire 
\ref{w4} implique
\begin{equation}\label{w.21}
|k^{\omega}-k^{0}|=\mathcal{O}(\frac{1}{h\sqrt{h}}\,h^{m-\alpha_{1}}\ln h^{-1}),\quad
l^{\omega}=l^{0}+\mathcal{O}(
\frac{1}{\sqrt{h}}\,h^{m-\alpha_{1}} \ln h^{-1}).
\end{equation}

On introduit la fonction holomorphe
\begin{equation}
F^{\omega}(w):=e^{\frac{l^{\omega}}{h}}
\det E_{-+}^{\omega}(w),\quad w\in W(w_{0}).
\end{equation}
Ce qui vient est une conséquence des propositions  \ref{w4}, \ref{w5bis}
et de (\ref{w.25}) :
%
%
%
%
%
\begin{corol} \label{w6}
Soit $w_{0}$ un point de $\Omega_{1}.$ Il existe un voisinage $W(w_{0})$ de 
$w_{0}$ inclus dans $\Omega_{1}$ et deux constantes positives $C$ et $\tilde{C}>0$ telles que
\\
(a) avec une probabilité $\ge  1- \gamma_{1}(h)$
nous avons
\begin{align}\label{w.23}
\ln|F^{\omega}(w)|&\le \frac{1}{h}(\mathrm{Re}\,l_{0}(w)+C\frac{1}{\sqrt{h}}h^{m-\alpha_{1}} \ln h^{-1}
+Ch\ln (h^{m-\alpha_{1}}\ln h^{-1})\nonumber\\
&:= \frac{1}{h}(\mathrm{Re}\,l_{0}(w)+ u(h))
\end{align}
pour tout $w$ dans $W(w_{0}),$ où $0<\gamma_{1}(h)$ tend vers zéro plus vite que n'importe quelle
puissance de $h.$ \\
(b) pour chaque $w$ de $W(w_{0}),$ et $\epsilon\in (0,m-\alpha_{1}-\rho-\frac{1}{4}),$
où $m-\alpha_{1}-\rho-\frac{1}{4}>0,$
nous avons 
\begin{align}\label{w.24}
\ln | F^{\omega}(w)|&\ge \frac{1}{h} ( \mathrm{Re}\,l_{0}(w)-C\frac{1}{\sqrt{h}}\,h^{m-\alpha_{1}}\ln h^{-1}
-Ch\ln h^{-1})\nonumber\\
&:=\frac{1}{h}(\mathrm{Re}\,l_{0}(w)-v(h))
\end{align}
avec une probabilité
$\ge 1- C h^{2\epsilon}.$
\end{corol}
%
%
%

On applique la proposition \ref{ss5}, avec  $f=F^{w},$ avec
$\tilde{\epsilon}= u(h)+v(h),$ et $\phi=\mbox{Re } l_{0}(w)+u(h).$
 Nous avons 
$\tilde{\epsilon}\asymp h\ln h^{-1},h\to 0$ puisque par hypothèse  
$m-\alpha_{1}-\rho-\frac{1}{4}>0$ et $\rho>1.$
(\ref{ss.28}) tient avec une probabilité comme dans $(a),$ (\ref{ss.30}) tient avec une probabilité
\[ \ge 1-C\frac{h^{2\epsilon}}{\sqrt{ h\ln \frac{1}{h}}}.\]
Ainsi donc, nous pouvons établir une version affaiblie des théorèmes
\ref{w1bis} et \ref{w2ter}, la condition (\ref{w.2}) étant remplacée par
\begin{equation}\label{w.25}
0<\epsilon<m-\alpha_{1}-\rho-\frac{1}{4}.
\end{equation}
%
%
%
%
%
\begin{theo}\label{w7}
On suppose l'hypothèse \ref{i10} vérifiée. 
Soit $\Gamma\subset\subset\Omega_{1}$ un ouvert à bord $C^{2}$ par morceaux, et  $\epsilon>0$  
vérifiant la condition (\ref{w.25}).
Il existe une constante  $C>0$ telle que  le nombre $N(T-\tilde{Q},\Gamma)$  
de valeur propre de $T-\tilde{Q}$
dans $\Gamma$ satisfait
\begin{equation}\label{w.26}
|N(T-\tilde{Q},\Gamma)-\frac{1}{2\pi h} \iint m_{\Gamma}\, dxd\xi | \le C
\frac{\sqrt{ h \ln\frac{1}{h}}}{h}
\end{equation}
avec une probabilité 
\[\ge 1-C\frac{h^{2\epsilon}}{\sqrt{h\ln\frac{1}{h}} }.\]
\end{theo}
%
%
\begin{theo}\label{w8}
Soit $\mathcal{G}$ une famille de domaines $\Gamma\subset\subset\Omega_{1},$
vérifiant les hypothèses du théorème \ref{ss8}. Nous supposons que l'hypothèse 
\ref{i10} est satisfaite. Choisissons $\epsilon$ comme dans le théorème \ref{w7},
alors avec une probabilité
\[\ge 1-C\frac{h^{2\epsilon}}{h\ln\frac{1}{h}},\]
nous avons (\ref{w.26}) avec une constante $C>0$ indépendante de $\Gamma.$
La probabilité est intéressante si $\epsilon> \frac{1}{2}.$
\end{theo}






